Concept Bottleneck Language Models For protein design

We introduce Concept Bottleneck Protein Language Models (CB-pLM), a generative masked language model with a layer where each neuron corresponds to an interpretable concept. Our architecture offers three key benefits: i) Control: We can intervene on concept values to precisely control the properties of generated proteins, achieving a 3 times larger change in desired concept values compared to baselines. ii) Interpretability: A linear mapping between concept values and predicted tokens allows transparent analysis of the model's decision-making process. iii) Debugging: This transparency facilitates easy debugging of trained models. Our models achieve pre-training perplexity and downstream task performance comparable to traditional masked protein language models, demonstrating that interpretability does not compromise performance. While adaptable to any language model, we focus on masked protein language models due to their importance in drug discovery and the ability to validate our model's capabilities through real-world experiments and expert knowledge. We scale our CB-pLM from 24 million to 3 billion parameters, making them the largest Concept Bottleneck Models trained and the first capable of generative language modeling.

==> discussion_conclusion.tex <==
% \begin{color}{myred}
\section{Discussion and Conclusion}
\subsection{Discussion}
In this paper, we applied our proposed architecture to masked language models for proteins. This versatile architecture can be adapted to any domain, such as NLP, by simply changing the training dataset, vocabulary, and concepts while keeping the model itself unchanged. Additionally, it can be easily adapted to other types of language models, such as autoregressive models, as demonstrated in Figure \ref{fig:autoregressive} in Appendix \ref{app:dis}. For autoregressive models, the embedding output from the transformer, typically used to predict the next token, is passed to the CB-layer to extract the known concept embedding and to an orthogonality network to extract the unknown concept embedding. These two embeddings are then concatenated and used to predict the next token.

An intuitive question that might arise is how we can control for new concepts. Specifically, if we are given a dataset with a new concept, can we fine-tune CB-LM to incorporate it? This can be achieved by creating a new CB-LM with an additional concept and copying the weights from the original model. In this setup, the only randomly initialized weights are for the new concept embedding  $e_{k+1}$, the concept classifier head for the new concept, and the linear decoder. The new model can then be trained to match the old model's concept output for existing concepts while aligning with the ground truth for the newly added concept.

In many real-world applications, we may need to generate sequences with previously unseen concepts or novel combinations of concepts not present in the training dataset. CB-LM provides this capability, as long as the new concepts can be expressed as functions of the existing ones. We demonstrate this capability in a toy task detailed in Appendix \ref{app:CB_plm_exp:more:OOD}, where we train a masked autoencoder vision transformer (MAE-ViT) \citep{he2022masked} with our architecture on a simple color-MNIST generation task. Our results show that the architecture can successfully generate blue-colored MNIST digits, despite the model never having encountered the color blue in the training dataset.

\section{Limitations}


One main limitation of CB-LM, similar to other concept bottleneck models \citep{ismail2023concept,koh2020concept}, is the requirement for the training dataset to be annotated with predefined concepts. Another drawback of our model is the necessity for unknown parts in the model embeddings. Generally, we believe this is unavoidable, as it is impractical to encode all the information needed for a generative task into a fixed number of predefined and interpretable concepts. Excluding unknown parts leads to unacceptable losses in task performance for generative models. However, this can pose challenges in terms of control and interpretability if the model relies on concept information from the unknown part. In the worst case, this could result in the model not using concept outputs at all. Our method takes steps to mitigate this issue, such as employing orthogonality loss, which helps improve control. Nonetheless, we acknowledge that some concept information remains in the unknown part, and developing better methods to disentangle this information would be desirable for the future.



\section{Conclusion}
We present Concept Bottleneck Language Models (CB-LM), a \textbf{\textit{controllable-interpretable-debuggable}} language model. We have demonstrated the effectiveness of our proposed architecture by applying it to masked protein language models. Our results show that this architecture can scale to large models, as evidenced by training Concept Bottleneck Protein Language Models (CB-pLM) with 24M, 150M, 650M, and 3B parameters to encode over 700 human-understandable concepts while maintaining pre-training perplexity comparable to traditional masked protein language models. Our findings indicate that CB-pLM offers superior control compared to conditional language models, along with interpretability and debugging capabilities. This work represents a significant step towards more interpretable, reliable, and debuggable neural networks.



% \begin{itemize}
%     \item Talk about how we can add new concepts.
%     \item Talk about how this can be used for other models in different domains.
%     \item limitations \tuomas{todo}
%     \begin{itemize}
%         \item Need of concepts and this can be addressed 
%         \item \nathan{inclusion of more complex concepts, e.g., those coming directly from wet lab experiments}
%         \item \nathan{discovering ``new" concepts from the unknown embeddings and thereby improving control by reducing the unknown embeddings; this i feel pretty optimistic about because we can "hold out" concepts and try to discover them, like they do in symbolic regression}
%         \item disentaglement.
%     \end{itemize}
% \end{itemize}
% \begin{color}{myred}
% \paragraph{Limitations:} One downside of our model is the need for unknown part in the model embeddings. In general, we think this is unavoidable as it is not possible to encode all information needed for a generative task into a fixed number of predefined and interpretable concepts, and not including unknown part leads to unacceptable losses task performance. However, this can cause problems in terms of control and interpretability, if the model also uses concept information from the unknown part, in the worst case leading the model to not using concept outputs at all.  Our method takes some steps towards mitigating this, such as the use of orthogonality loss, which helps improve the control, but we know some concept information does remain in the unknown part, and better methods to disentangle this would be desirable for the future.
% \end{color}

